TrustNet: Learning from Trusted Data Against (A)symmetric Label Noise

Robustness to label noise is a critical property for weakly-supervised classifiers trained on massive datasets. Robustness to label noise is a critical property for weakly-supervised classifiers trained on massive datasets. In this paper, we first derive analytical bound for any given noise patterns. Based on the insights, we design TrustNet that first adversely learns the pattern of noise corruption, being it both symmetric or asymmetric, from a small set of trusted data. Then, TrustNet is trained via a robust loss function, which weights the given labels against the inferred labels from the learned noise pattern. The weight is adjusted based on model uncertainty across training epochs. We evaluate TrustNet on synthetic label noise for CIFAR-10 and CIFAR-100, and real-world data with label noise, i.e., Clothing1M. We compare against state-of-the-art methods demonstrating the strong robustness of TrustNet under a diverse set of noise patterns.

==> loss.tex <==
\% This should be comment for main paper!
In this Section, we present the related work loss functions. 
\subsection{Symmetric Cross Entropy}
Based on ~\cite{wang2019symmetric}, the loss function shows a Symmetric Cross Entropy which is inspired by symmetric KL-divergence. 


\begin{equation} \label{eq:6}
\begin{split}
   \mathcal{L}_{total} = \alpha \times -\frac{1}{n}\sum_{i=1}^n\boldsymbol{y}_i\log \mathcal{F}(\mathcal{\theta}, \boldsymbol{x}_i) + \\
   \beta \times -\frac{1}{n}\sum_{i=1}^n\mathcal{F}(\mathcal{\theta}, \boldsymbol{x}_i)\log \boldsymbol{y}_i
   \end{split}
\end{equation}

where $\alpha$ and $\beta$ are weights of cross-entropy loss functions. 

\subsection{D2L}
D2L loss function ~\cite{ma2018dimensionality} is a weighted average which Local Intrinsic Dimensionality
score is an estimation for weights of predicted and given labels. The estimation of LID score which is formulated: 
\begin{equation} \label{eq:7}
\begin{split}
   \hat{LID}(x, X_B) =  -(\frac{1}{k}\sum_{i=1}^k \log \frac{r_i(g(x),g(X_B))}{r_{max}(g(x),g(X_B)})^{-1}
   \end{split}
\end{equation}

where $g(.)$ is the output of the second-to-last layer of the network, $r_i(g(x),g(X_B))$ is the distance of $g(x)$ to its $i$-th nearest neighbour in the transformed set $g(X_B)$, and $r_{max}$ represents the radius of the neighborhood. 
To train a Deep Neural network with noisy labels, they propose to reduce the effort of noisy labels on learning the true data distribution using the following adaptive LID-corrected labels:
\begin{equation} \label{eq:8}
\begin{split}
   y^* = \alpha_i y + (1 - \alpha_i) \hat{y}
   \end{split}
\end{equation}

where $\alpha_i$ is a LID-based factor that updates at the $i$-th training epoch:
\begin{equation} \label{eq:9}
\begin{split}
   \alpha_i = \exp(-\lambda \frac{\hat{LID}_i}{\min_{j=0}^{i-1}\hat{LID}_j})
   \end{split}
\end{equation}

where $\lambda = \frac{i}{T}$ is a weighting that indicates decreasing confidence in the raw labels when the training proceeds to the dimensionality expansion stage (that is, when LID begins to increase). The training loss can then be refined as:

\begin{equation} \label{eq:10}
\begin{split}
   \mathcal{L}_{total} = -\frac{1}{n}\sum_{i=1}^n\boldsymbol{y}_i^*\log \mathcal{F}(\mathcal{\theta}, \boldsymbol{x}_i)
   \end{split}
\end{equation}

\subsection{Forward}
Other modification in loss function is performed by estimating transition matrix between noisy labels and clean labels. In ~\cite{patrini2017making}, they find noise transition matrix and update loss function which is formulated by

\begin{equation} \label{eq:11}
\begin{split}
   \mathcal{L}_{total} = -\frac{1}{n}\sum_{i=1}^n\boldsymbol{y}_i\log (\boldsymbol{T}_i^T . \mathcal{F}(\mathcal{\theta}, \boldsymbol{x}_i))
   \end{split}
\end{equation}

where $T$ is the transition matrix which is defined by 
\begin{equation} \label{eq:12}
\begin{split}
   T_{i,j} = p(\boldsymbol{y}_j | \boldsymbol{y}_i)
   \end{split}
\end{equation}

$p(.)$ is the probability of changing true label to noisy label.
\subsection{Bootstrap}
Reed et al. ~\cite{reed2014training} proposed a weighted average of raw labels and their predicted labels. The loss function equal to:

\begin{equation} \label{eq:13}
\begin{split}
   \mathcal{L}_{total} = -\frac{1}{n}\sum_{i=1}^n (\alpha \boldsymbol{y}_i + (1 - \alpha) \mathcal{F}(\mathcal{\theta}, \boldsymbol{x}_i)) \log \mathcal{F}(\mathcal{\theta}, \boldsymbol{x}_i) 
   \end{split}
\end{equation}

where $\alpha$ is the weight factor. 

==> noise_old.tex <==
In this section, we present theoretical bound on test accuracy of deep neural networks that are assumed to have high learning capacity. Here test accuracy is defined as the probability that the predicted label $\hat{y}$ is equal to the given label $y$. We first summarize prior results~\cite{chen:2019:ICML:understanding} which derive the bound for a restricted subset of noise patterns and then derive a general bound valid for any given noise distribution. We apply our general formulation to derive the bounds for \rb{XXX} exemplary cases: partial noisy patterns and targeted noisy patterns \rb{review list}. These patterns are more complex than the prior art patterns. \rb{why?}
% first present the prior theoretical result on noisy impact. We then extend such bound to fully asymmetric noise, which is more complicated than noise pattern studied in the prior art.  
% \lc{In the following: lets first show the noise pattern by the confusion matrix ( transition matrix), and then theoretical bounds}
\subsection{Preliminaries}
Consider the classification problem having dataset $\mathcal{D} = \{(\boldsymbol{x}_1,  \boldsymbol{y}_1),  (\boldsymbol{x}_2,  \boldsymbol{y}_2), ... , (\boldsymbol{x}_N, \boldsymbol{y}_N) \}$ where $\boldsymbol{x}_k$ denotes the $k^{th}$ observed sample, and $\boldsymbol{y}_k \in \{0,1\}^C$ the corresponding label vectors over $C$ classes representing the noisy given classes. Besides, for small subset of $\mathcal{D}$, In addition to the $\boldsymbol{y}_k$  for each sample, the ground truth is available where $\boldsymbol{t}_k \in \{0,1\}^C$ which is in the same format as $\boldsymbol{y}_k$ corresponding true labels. Also, assume that new training set $\mathcal{T} = \{(\boldsymbol{x}_1,  \boldsymbol{y}_1, \boldsymbol{t}_1), (\boldsymbol{x}_2,  \boldsymbol{y}_2, \boldsymbol{t}_2), ... , (\boldsymbol{x}_M, \boldsymbol{y}_M, \boldsymbol{t}_M)\}$ where $M$ denotes the number of samples in new training set which $M < N$.
Traditional classification problems only use the sample $\boldsymbol{x}_k$ and its true label $\boldsymbol{t}_k$. Let $\hat{y}$ denote the true label and $\mathbf{T}_{ij} = P(y = j | \hat{y} = i)$ describe the noise transition matrix. $\varepsilon$ denotes noise ratio. Let $f(x; \theta)$ denote a neural network parameterized by $\theta$, and $y^f \in [C]$ denote the predicted label of $x$ given by the network $f(x; \theta)$.
\subsection{Prior Results}
Prior art studied the theoretical bounds on test accuracy for: (i) symmetric noise: a given class label is altered to another class label following uniform distribution with equal probabilities; and (ii) targeted asymmetric noise: each class label is swapped with a specific other class label only (adjacent class label in the example). Fig.~\ref{fig:cm_types}(a)-(c) illustrates the confusion matrices resulting from these three noise patterns on CIFAR-10 with a noise ratio of $0.4$. 
Fig~\ref{subfig:clothing1m}, shows the confusion matrix of real world noisy data which is Clothing1M. 

% (ii) partial asymmetric noise: only some classes are affected by bimodal noise;

\begin{figure*}[th]
	\centering
	{
	\subfloat[Symmetric noise]{
	    \label{subfig:cm_symmetric}
	    \includegraphics[width=0.25\linewidth]{figures/TM_sym.pdf}}
% 	\subfloat[Partial asymmetric noise]{
% 	    \label{subfig:cm_asymmetric_p}
% 	    \includegraphics[width=0.32\linewidth]{figures/TM_asymp.pdf}}
	\subfloat[Targeted noise]{
	    \label{subfig:cm_asymmetric_f}
	    \includegraphics[width=0.25\linewidth]{figures/TM_asymf.pdf}}
	\subfloat[Clothing1M noise]{
	    \label{subfig:clothing1m}
	    \includegraphics[width=0.25\linewidth]{figures/clothing1m.pdf}}
	\subfloat[Theoretical bound]{
	    \label{subfig:acc_types}
	    \includegraphics[width=0.25\linewidth]{figures/allbounds.pdf}}
	}
	\caption{Examples of noise transition matrix $\mathbf{T}$ taking CIFAR-10 with 10 classes and 40\% noise ratio. \rb{remove partial asymmetric noise bound from figure}}
	\label{fig:cm_types}
\end{figure*}

\subsection{General accuracy bound}

\begin{lemma}\label{th:general}
For asymmetric noise with any distribution of ratio $\varepsilon$, the test accuracy is

\begin{equation} \label{eq:asymn}
\begin{split}
   P(\hat{y} = y) = \sum_i(1 - \varepsilon_i)^2 + \sum_i{\varepsilon_i^2} \sum_{j=1}^{C-1}{P^2(y = j)}
   \end{split}
\end{equation}
\end{lemma}
\begin{proof}
we have
\[T_{ij} = P(y = j |  \hat{y} = i) = P(y = \hat{y}) + P(y \neq \hat{y})\]
we know that $T_{ij}$ when $i = j$ equals to $1 - \varepsilon$. In addition, for $i \neq j$, we have
\[T_{ij} = \varepsilon P(y = j)\] 
where it derives from the probability of selecting other labels($\varepsilon$) multiplication in the probability of change to $j$ (P(y = j)). %Because the probability can come from any distribution such as normal distribution which in this case, P(y = x) equals to
%\[P(y = x) = \int_{x}^{x+dx} \frac{1}{\sqrt{2\pi}\sigma} e^{\frac{-(x - \mu)^2}{2\sigma^2}} dx\]

now, we have

\begin{equation} \label{eq:t1matri}
\begin{split}
   P(y^f = y) = \sum_{i=1}^C{P(\hat{y} = i) P(y^f = y | \hat{y} = i)} = \sum_{i=1}^C{P(\hat{y} = i)}\sum_{j=1}^C{T^2_{ij}}. \\
   P(y^f = y) = \sum_{i=1}^C{P(\hat{y} = i)}[T^2_{ii} + \sum_{j \neq i}^{C}{T^2_{ij}}] \\
   = \sum_{i=1}^C{P(\hat{y} = i)}[(1 - \varepsilon)^2 + \varepsilon^2 \sum_{j \neq i}^{C}{P^2(y = j)}]\\
   = (1 - \varepsilon)^2 + \varepsilon^2 \sum_{i=1}^C{P(\hat{y} = i)} \sum_{j \neq i}^{C}{P^2(y = j)}
   \end{split}
\end{equation}
\end{proof}



%\begin{lemma}

%For symmetric noise of ratio $\mathcal{\varepsilon}$, the test accuracy is 
%\begin{equation} \label{eq:symnoise}
%\begin{split}
%   P(y^f = y) = {(1 - \varepsilon)}^2 + \frac{\varepsilon^2}{c - 1}
%   \end{split}
%\end{equation}
%\end{lemma}

%\begin{lemma}
%For asymmetric noise of ratio $\varepsilon$, the test accuracy is 
%\begin{equation} \label{eq:asymfnoise}
%\begin{split}
 %  P(y^f = y) = {(1 - \varepsilon)}^2 + \varepsilon^2
%  \end{split}
%\end{equation}
%\end{lemma}

%According to~\cite{chen:2019:ICML:understanding}, we have
%\begin{equation} \label{eq:tmatrix}
%\begin{split}
 %  P(y^f = y) = \sum_{i=1}^c{P(\hat{y} = i) P(y^f = y | \hat{y} = i)}
 %  = \sum_{i=1}^c{P(\hat{y} = i)}\sum_{j=1}^c{T^2_{ij}}
 %  \end{split}
%\end{equation}

\subsubsection{Partial targeted}
In this pattern only a subset $S$ of label classes is affected by targeted noise. \rb{which type? Example figure 1b}

\begin{lemma}\label{th:partial}
For partial asymmetric noise with ratio $\varepsilon$, where $S$ is the  selected labels set for flipping and $U$ is the unselected labels set, the test accuracy is
\begin{equation} \label{eq:asymp}
\begin{split}
   P(y^f = y) = \frac{|S|}{C}({(1 - \varepsilon)}^2 + \varepsilon^2) + \frac{|U|}{C}
   \end{split}
\end{equation}
\end{lemma}

\begin{proof}

we have

\begin{equation} \label{eq:tmatri}
\begin{split}
   P(y^f = y) = \sum_{i=1}^C{P(\hat{y} = i) P(y^f = y | \hat{y} = i)} = \sum_{i=1}^C{P(\hat{y} = i)}\sum_{j=1}^C{T^2_{ij}} \\
   = \sum_{i=1}^{|S|}{P(\hat{y} = i) P(y^f = y | \hat{y} = i)} + \sum_{i'=1}^{|U|}{P(\hat{y} = i') P(y^f = y | \hat{y} = i')} \\
   \sum_{i=1}^{|S|}{P(\hat{y} = i)} \sum_{j=1}^C{T^2_{ij}} + \sum_{i'=1}^{|U|}{P(\hat{y} = i')} \sum_{j'=1}^c{T^2_{i'j'}} \\
   = ((1 - \varepsilon)^2 + \varepsilon^2) \sum_{i=1}^{|S|}{P(\hat{y} = i)} + \sum_{i'=1}^{|U|}{P(\hat{y} = i')}\\
   = \frac{|S|}{C}({(1 - \varepsilon)}^2 + \varepsilon^2) + \frac{|U|}{C}
   \end{split}
\end{equation}
\end{proof}

\subsubsection{General relation between test accuracy and noise ratio for asymmetric}

\begin{figure*}[th]
	\centering
	{
%	\subfloat[$\mu = 0.2$,$\sigma = 0.05$]{
%	    \label{subfig:cm_normal_m2_v0.05}
%	    \includegraphics[width=0.33\linewidth]{normal_m2_v0-05.pdf}}
	\subfloat[$\mu = 0.1$,$\sigma = 0.05$]{
	    \label{subfig:cm_normal_m5_v0.05}
	    \includegraphics[width=0.25\linewidth]{figures/nor_m01_v005.pdf}}
	\subfloat[$\mu = 0.1$,$\sigma = 0.5$]{
	    \label{subfig:cm_normal_m5_v0.05}
	    \includegraphics[width=0.25\linewidth]{figures/nor_m01_v05.pdf}} 
	\subfloat[$\mu = 0.1$,$\sigma = 1$]{
	    \label{subfig:cm_normal_m2_v1}
	    \includegraphics[width=0.25\linewidth]{figures/nor_m01_v1.pdf}}
	\subfloat[$\mu = 0.1$,$\sigma = 10$]{
	    \label{subfig:cm_normal_m5_v10}
	    \includegraphics[width=0.25\linewidth]{figures/nor_m01_v10.pdf}}
%	\subfloat[$\mu = 0.5$,$\sigma = 100$]{
%	    \label{subfig:cm_normal_m5_v100}
%	    \includegraphics[width=0.33\linewidth]{normal_m5_v100.pdf}}
	}
	\caption{Examples of noise transition matrix $\mathbf{T}$ taking CIFAR-10 with 10 classes and noise ratio 0.4 for Gaussian distribution with different $\mu, \sigma$.}
	\label{fig:cm_normal}
\end{figure*}


\begin{figure*}[th]
	\centering
	{
%	\subfloat[$\mu = 0.2$,$\sigma = 0.05$]{
%	    \label{subfig:cm_normal_m2_v0.05}
%	    \includegraphics[width=0.33\linewidth]{normal_m2_v0-05.pdf}}
	\subfloat[$\mu_1 = 0.2,\sigma_1 = 0.05,\mu_2 = 0.7,\sigma_2 = 0.5$]{
	    \label{subfig:cm_bimodal_m102_m207}
	    \includegraphics[width=0.25\linewidth]{figures/cm_bimodal_m102_v1005_m207_v205.pdf}}
	\subfloat[$\mu_1 = 0.2,\sigma_1 = 0.05,\mu_2 = 0.7,\sigma_2 = 0.05$]{
	    \label{subfig:cm_normal_m5_v0.05}
	    \includegraphics[width=0.25\linewidth]{figures/cm_bimodal_m102_v1005_m207_v2005.pdf}} 
	\subfloat[Theoretical bound]{
	    \label{subfig:acc_types}
	    \includegraphics[width=0.25\linewidth]{figures/theoall.pdf}}
% 	\subfloat[$\mu = 0.1$,$\sigma = 1$]{
% 	    \label{subfig:cm_normal_m2_v1}
% 	    \includegraphics[width=0.25\linewidth]{figures/nor_m01_v1.pdf}}
% 	\subfloat[$\mu = 0.1$,$\sigma = 10$]{
% 	    \label{subfig:cm_normal_m5_v10}
% 	    \includegraphics[width=0.25\linewidth]{figures/nor_m01_v10.pdf}}
%	\subfloat[$\mu = 0.5$,$\sigma = 100$]{
%	    \label{subfig:cm_normal_m5_v100}
%	    \includegraphics[width=0.33\linewidth]{normal_m5_v100.pdf}}
	}
	\caption{Examples of noise transition matrix $\mathbf{T}$ taking CIFAR-10 with 10 classes and noise ratio 0.4 for bimodal normal distribution (with two peaks at class 2 and class 7).}
	\label{fig:cm_normal}
\end{figure*}


 %= (1 - \varepsilon)^2 + \varepsilon^2 \sum_{j \neq i}^{c}{P^2(y = j)}

% \begin{table}[t]
%     \centering
%     \caption{Notation}
%     \begin{tabular}{|c|l|}
%     \hline
%       $\boldsymbol{\hat{y}}$ & original label\\ \hline
%       $\boldsymbol{y}$ & given label\\ \hline
%       $\boldsymbol{y}^f$ & predicted label\\ \hline
%       $T_{i,j}$ & Confusion matrix\\ \hline
%       $\varepsilon$ &  Noise ratio\\ \hline
%       $c$ &  number of classes\\ \hline
%     \end{tabular}
%     \label{tab:my_label}
% \end{table}



Figure~\ref{fig:theovsemp}, demonstrates the theoretical result for different types of noise.  



\subsection{Empirical validation and analysis}

In the following, we present new type of asymmetric noise which is derived from Gaussian distribution. 



\begin{figure*}[th]
	\centering
	{
	\subfloat[Partial asymmetric]{
	    \label{subfig:acc_theoemp}
	\includegraphics[width=0.33\linewidth]{figures/parTheoEmp.pdf}
	}
	  \subfloat[Asymmetric Normal]{%mu = 0.1, var = 1
	    \label{subfig:acc_theoemp}
	    \includegraphics[width=0.33\linewidth]{figures/norm_TheoEmp.pdf}}
	   \subfloat[Asymmetric Bimodal]{%mu1 = 0.2, var1 = 0.5, mu2 = 0.7, var2 = 1
	    \label{subfig:acc_theoemp}
	    \includegraphics[width=0.33\linewidth]{figures/TheoEmpBimodal.pdf}}
}
	\caption{Validation on CIFAR-10: analytical results v.s. empirical accuracy with different noise ratios}
	\label{fig:theovsemp}
\end{figure*}


\begin{figure*}[th]
	\centering
	{
   \subfloat[Different $\mu,\sigma=0.5$]{
	    \label{subfig:diffmean}
	    \includegraphics[width=0.33\linewidth]{figures/normal_dif_mean.pdf}}
    \subfloat[Different $\sigma,\mu=0.9$]{
	    \label{subfig:diffvar}
	    \includegraphics[width=0.33\linewidth]{figures/normal_dif_var.pdf}}
	 \subfloat[Bimodal distribution]{
	    \label{subfig:acc_types}
	    \includegraphics[width=0.33\linewidth]{figures/otherDis.pdf}}
}
	\caption{Analytical results: the impact of noise patterns on the test accuracy with respect to different noise ratios}
	\label{fig:theovsemp}
\end{figure*}




